DAFNE and KLOE-2

The DAFNE collider, located in the Frascati National Laboratories of INFN, has two main rings, where electrons and positrons are stored to collide at a center of mass energy of 1.02 GeV, the phi resonance mass. KLOE-2 experiment is located at the collider interaction region. The detector is capable to observe and collect data coming from phi decay: charged and neutral kaon pairs, lighter unflavored mesons (eta, eta', f0, a0, omega/rho). In the first half of 2013 the KLOE detector has been upgraded inserting new detector layers in the inner part of the apparatus, around the interaction region in order to improve detector hermeticity and acceptance. The long shutdown has been used to undertake a general consolidation program aimed at improving the DAFNE performances. This contribution presents the phi-factory setup and the achieved performances in terms of beam currents, luminosity and related aspects together with the KLOE-2 physics program, upgrade status report and recent physics results.

==> ads_def.tex <==
%
% A.De Santis Definitions
%

% typesetting & referencing
\def\ifm#1{\relax\ifmmode#1\else$#1$\fi}
\newcommand{\refeq}[1]{(\ref{#1})}
\def\fig#1{fig.~\ref{#1}}
\def\Fig#1{Fig.~\ref{#1}}
\def\tab#1{tab.~\ref{#1}}
\def\Tab#1{Tab.~\ref{#1}}
\def\equ#1{eq.~\ref{#1}}
\def\Equ#1{Eq.~\ref{#1}}
\def\etal{{\it et al.}}
\def\red{\color{red}}
\def\blue{\color{blue}}
\def\green{\color{green}}
\renewcommand{\bold}[1]{{\bfseries {#1}}}

% shortcuts for phys
\def\f{\ifm{\phi}}    
\def\ff{\f--factory}
\def\epm{\ifm{e^+e^-}}
\renewcommand{\to}{\ensuremath{\rightarrow}}
\def\dafne{DA$\Phi$NE}
\def\ep{\ifm{e^+}}
\def\el{\ifm{e^-}}
\def\ks{\ifm{K_S}}
\def\kl{\ifm{K_L}}
\def\ko{\ifm{K_0}}
\def\ok{\ifm{\overline{K}_0}}
\def\kp{\ifm{K^+}}
\def\km{\ifm{K^-}}
\def\pip{\ifm{\pi^+}}
\def\pim{\ifm{\pi^-}}
\def\pio{\ifm{\pi^0}}
\def\JPC{\ifm{J^{PC}}}
\def\CP{\ifm{CP}}
\def\CPT{\ifm{CPT}}
\def\kltre{\ifm{\mbox{K}_\ell3}}
\def\kmutre{\ifm{\mbox{K}_\mu3}}
\def\ketre{\ifm{\mbox{K}_e3}}


%shotrcuts for math 
\def\ab{\ifm{\sim}}
\newcommand{\ket}[1]{\ifm{|#1\rangle}}
\newcommand{\braket}[2]{\ifm{\langle #1|#2 \rangle}}
\def\order#1,{\ifm{\mathcal{O}(10^{#1})}}
\def\x{\ifm{\times}}

%shortcuts for units
\def\MeV{\ifm{\mbox{MeV}}}
\def\GeV{\ifm{\mbox{GeV}}}
\def\mum{\ifm{\mbox{$\mu$m}}}
\def\mm{\ifm{\mbox{mm}}}
\def\mub{\ifm{\mbox{$\mu$b}}}
\def\invfb{\ifm{\mbox{fb}^{-1}}}
\def\invpb{\ifm{\mbox{pb}^{-1}}}
\def\cms{\ifm{\mbox{cm}^{-2}}\mbox{s}^{-1}}


%shortcuts for Lorentz

\def\Dt{\ifm{\Delta \tau}}
\def\Ts{\ifm{{T_{sid}}}}
\def\Tsb{\ifm{\{T_{sid}\}}}
\def\Damu{\ifm{\Delta a_\mu}}
\def\Dax{\ifm{\Delta a_X}}
\def\Day{\ifm{\Delta a_Y}}
\def\Daz{\ifm{\Delta a_Z}}
\def\Dao{\ifm{\Delta a_0}}

